Enhancing TTS Stability in Hebrew using Discrete Semantic Units

This study introduces a refined approach to Text-to-Speech (TTS) generation that significantly enhances sampling stability across languages, with a particular focus on Hebrew. By leveraging discrete semantic units with higher phonetic correlation obtained from a self-supervised model, our method addresses the inherent instability often encountered in TTS systems, especially those dealing with non-diacriticized scripts like Hebrew. Utilizing HuBERT codes, our model generates discrete representations that are optimized for TTS tasks, thereby reducing the dependency on diacritic-based text processing. This advancement not only simplifies the language modeling process but also improves the robustness and shows controllability of the speech output due to disentenglement properties of the semantic units. The inclusion of a speaker embedding in the vocoder further aids in capturing the unique vocal characteristics of the speaker, contributing to the naturalness of the synthesized speech. Our experimental results demonstrate that this approach not only maintains high performance in Hebrew but also shows adaptability to English, underscoring its effectiveness in enhancing stability in TTS systems universally. Our method, named LOTHM (Language of The Hebrew Man), outperforms existing methods in terms of stability while achieving naturalness and speaker similarity on par with previous methods, making it a compelling choice for future speech synthesis applications. Samples can be found in our page pages.cs.huji.ac.il/adiyoss-lab/LoTHM .

==> figs/boxplot.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{image.png}
    \caption{Enter Caption}
    \label{fig:enter-label}
\end{figure}

==> figs/corr_speaking_rate.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{image.png}
    \caption{Enter Caption}
    \label{fig:enter-label}
\end{figure}

==> tables/eng_valle.tex <==
\begin{table}[]
\begin{tabular}{lll}
        & WER           & CER           \\ \hline
EnCodec (x1) & 0.397         & 1.29          \\
HuBERT (x1)  & 0.14 & 0.08 \\ \hline
HuBERT (x3)  & \textbf{0.08} & \textbf{0.04} \\ \hline
GT      & 0.03          & 0.008         \\ \hline
\end{tabular}
\end{table}

==> tables/mos.tex <==
\begin{table}[h!]
\centering
\caption{Evaluation Metrics Summary}
\begin{tabular}{|l|l|c|c|}
\hline
\textbf{Metric} & \textbf{Model} & \textbf{Mean} & \textbf{Std. Dev.} \\ \hline
\multirow{5}{*}{\textbf{Naturalness}} & GT & 4.83 & 0.43 \\ 
 & Valle & 3.92 & 1.17 \\ 
 & Ours & 4.01 & 0.96 \\ 
 & MMS & 2.54 & 1.14 \\ 
 & RoboShaul & 3.52 & 1.24 \\ \hline
\multirow{5}{*}{\textbf{Text Accuracy}} & GT & 4.72 & 0.62 \\ 
 & Valle & 4.27 & 0.97 \\ 
 & Ours & 4.48 & 0.80 \\ 
 & MMS & 2.31 & 0.96 \\ 
 & RoboShaul & 4.17 & 0.88 \\ \hline
\multirow{3}{*}{\textbf{Speaker Resemblance (Valle vs Ours vs Shaul)}} & Ours & 3.21 & 1.28 \\ 
 & Valle & 2.55 & 1.27 \\ 
 & RoboShaul & 2.82 & 1.24 \\ \hline
\multirow{2}{*}{\textbf{Speaker Resemblance (Valle vs Ours)}} & Ours & 3.28 & 1.22 \\ 
 & Valle & 3.45 & 1.12 \\ \hline
\textbf{Speaker Resemblance (Ours using a different prompt)} & Ours & 2.55 & 1.20 \\ \hline
\end{tabular}
\label{table:evaluation_summary}
\end{table}


==> tables/table_mos_and_wer.tex <==
% \begin{table*}[t!]
%     % \begin{strip}
%     \centering
%     \caption{Results of Human Evaluation}
%     \resizebox{1.5\columnwidth}{!}{
%     \begin{tabular}{@{}l|ccc|ccc@{}}
%     \toprule
%     \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{Objective Metrics}} & \multicolumn{3}{c}{\textbf{Human Study}} \\ \cmidrule(l){2-7}
%     & \textbf{WER$\downarrow$} & \textbf{CER$\downarrow$} & \textbf{Spk. Sim.$\uparrow$} & \textbf{Naturalness$\uparrow$} & \textbf{Content$\uparrow$} & \textbf{Spk. Sim.$\uparrow$} \\
%     \midrule
%     \textbf{Reference} & 0.07 & \textbf{0.03} & 0.96 & 4.81 ($\pm$0.44) & 4.73 ($\pm$0.51) & - \\
%     \midrule
%     \textbf{MMS} & 0.23 & 0.07 & - & 2.55 ($\pm$1.15) & 2.27 ($\pm$0.91) & - \\
%     \textbf{Overflow} & 0.20 & 0.08 & 0.81 & 3.57 ($\pm$1.16) & 4.16 ($\pm$0.86) & 2.71 ($\pm$1.25) \\
%     \textbf{Ours (sampled once)} & 0.17 & 0.09 & 0.93 & \textbf{3.97} ($\pm$1.06) & \textbf{4.44} ($\pm$0.88) & 3.11 ($\pm$1.27) \\
%     \textbf{Ours (sampled 3 times)} & \textbf{0.10} & \textbf{0.03} & - & - & - & - \\
%     \textbf{HebTTS (sampled once)} & 0.34 & 0.18 & 0.85 & 3.97 ($\pm$1.12) & 4.31 ($\pm$0.94) & 2.95 ($\pm$1.30) \\
%     \textbf{HebTTS (sampled 3 times)} & 0.19 & 0.08 & - & - & - & - \\
%     \bottomrule
%     \end{tabular}}
%     % \end{strip}
% \end{table*}

% \begin{table*}[t!]
%   \label{tab:main-wer}
%   \centering
%     \caption{Results of Human Evaluation}
%     \resizebox{0.9\textwidth}{!}{
%     \begin{tabular}{@{}l|ccc|ccc@{}}
%     \toprule
%     \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{Objective Metrics}} & \multicolumn{3}{c}{\textbf{Human Study}} \\ \cmidrule(l){2-7}
%     & \textbf{WER$\downarrow$} & \textbf{CER$\downarrow$} & \textbf{Spk. Sim.$\uparrow$} & \textbf{Naturalness$\uparrow$} & \textbf{Content$\uparrow$} & \textbf{Spk. Sim.$\uparrow$} \\
%     \midrule
%     \textbf{Reference} & 0.07 & \textbf{0.03} & 0.96 & 4.81 ($\pm$0.44) & 4.73 ($\pm$0.51) & - \\
%     \midrule
%     \textbf{MMS} & 0.23 & 0.07 & - & 2.55 ($\pm$1.15) & 2.27 ($\pm$0.91) & - \\
%     \textbf{Overflow} & 0.20 & 0.08 & 0.81 & 3.57 ($\pm$1.16) & 4.16 ($\pm$0.86) & 2.71 ($\pm$1.25) \\
%     \textbf{Ours (sampled once)} & 0.17 & 0.09 & 0.93 & \textbf{3.97} ($\pm$1.06) & \textbf{4.44} ($\pm$0.88) & 3.11 ($\pm$1.27) \\
%     \textbf{Ours (sampled 3 times)} & \textbf{0.10} & \textbf{0.03} & - & - & - & - \\
%     \textbf{HebTTS (sampled once)} & 0.34 & 0.18 & 0.85 & 3.97 ($\pm$1.12) & 4.31 ($\pm$0.94) & 2.95 ($\pm$1.30) \\
%     \textbf{HebTTS (sampled 3 times)} & 0.19 & 0.08 & - & - & - & - \\
%     \bottomrule
%     \end{tabular}}
% \end{table*}


% \begin{table*}[t!]
% \centering
% \caption{Results of Human Evaluation}
% \resizebox{0.9\textwidth}{!}{
% \begin{tabular}{@{}l|ccc|ccc@{}}
% \toprule
% \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{Objective Metrics}} & \multicolumn{3}{c}{\textbf{Human Study}} \\ \cmidrule(l){2-7}
% & \textbf{WER$\downarrow$} & \textbf{CER$\downarrow$} & \textbf{Spk. Sim.$\uparrow$} & \textbf{Naturalness$\uparrow$} & \textbf{Content$\uparrow$} & \textbf{Spk. Sim.$\uparrow$} \\
% \midrule
% \textbf{Reference} & 0.07 & \textbf{0.03} & 0.96 & 4.81 ($\pm$[4.73921429 4.87920631]) & 4.74 ($\pm$[4.65582848 4.81785583]) & - \\
% \midrule
% \textbf{MMS} & 0.23 & 0.07 & - & 2.56 ($\pm$[2.37437918 2.74404189]) & 2.28 ($\pm$[2.1342802 2.4315095]) & - \\
% \textbf{Overflow} & 0.20 & 0.08 & 0.81 & 3.57 ($\pm$[3.38855778 3.75617899]) & 4.16 ($\pm$[4.02747097 4.3014761 ]) & 3.57 ($\pm$[3.38855778 3.75617899]) \\
% \textbf{Ours (sampled once)} & 0.17 & 0.09 & 0.93 & 3.95 ($\pm$[3.78450473 4.12338988]) & \textbf{4.44} ($\pm$[4.30103621 4.58054318]) & 3.95 ($\pm$[3.78450473 4.12338988]) \\
% \textbf{Ours (sampled 3 times)} & \textbf{0.10} & \textbf{0.03} & - & - & - & - \\
% \textbf{HebTTS (sampled once)} & 0.34 & 0.18 & 0.85 & \textbf{3.96} ($\pm$[3.78289862 4.13815384]) & 4.31 ($\pm$[4.15968575 4.45873486]) & 3.96 ($\pm$[3.78289862 4.13815384]) \\
% \textbf{HebTTS (sampled 3 times)} & 0.19 & 0.08 & - & - & - & - \\
% \bottomrule
% \end{tabular}}
% \end{table*}
\begin{table*}
\label{tab:main-wer}

\centering
\caption{Results of Human Evaluation}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{@{}l|ccc|ccc@{}}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{Objective Metrics}} & \multicolumn{3}{c}{\textbf{Human Study}} \\ \cmidrule(l){2-7}
& \textbf{WER$\downarrow$} & \textbf{CER$\downarrow$} & \textbf{Spk. Sim.$\uparrow$} & \textbf{Naturalness$\uparrow$} & \textbf{Content$\uparrow$} & \textbf{Spk. Sim.$\uparrow$} \\
\midrule
\textbf{Reference} & 0.07 & \textbf{0.03} & 0.96 & 4.81 $\pm$0.07 & 4.74 $\pm$0.08 & - \\
\midrule
\textbf{MMS} & 0.23 & 0.07 & - & 2.56 $\pm$0.18 & 2.28 $\pm$0.15 & - \\
\textbf{Overflow} & 0.20 & 0.08 & 0.81 & 3.57 $\pm$0.18 & 4.16 $\pm$0.14 & 2.75 $\pm$0.22 \\
\textbf{Ours (sampled once)} & 0.17 & 0.09 & 0.93 & 3.95 $\pm$0.17 & \textbf{4.44} $\pm$0.14 & 3.10 $\pm$0.15 \\
\textbf{Ours (sampled 3 times)} & \textbf{0.10} & \textbf{0.03} & - & - & - & - \\
\textbf{HebTTS (sampled once)} & 0.34 & 0.18 & 0.85 & \textbf{3.96} $\pm$0.18 & 4.31 $\pm$0.15 & 2.95 $\pm$0.16 \\
\textbf{HebTTS (sampled 3 times)} & 0.19 & 0.08 & - & - & - & - \\
\bottomrule
\end{tabular}}
\end{table*}

==> tables/wer_cer.tex <==
\begin{table}[h]
\centering
\caption{Comparison of Objective Metrics and Human Evaluation}
\label{tab:metrics_evaluation}
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{@{}c|ccc|ccc@{}}
\toprule
                         & \multicolumn{3}{c|}{\textbf{Objective Metrics}} & \multicolumn{3}{c|}{\textbf{Human Evaluation}} \\ \midrule
Model                    & WER          & CER          & Spk. Sim.         & Naturalness     & Content     & Spk. Sim.     \\ \midrule
Reference                &              &              &                   &                 &             &               \\ \midrule
HebTTS (sampled once)    &              &              &                   &                 &             &               \\
HebTTS (sampled 3 times) &              &              &                   &                 &             &               \\
Ours (sampled once)      &              &              &                   &                 &             &               \\
Ours (samples 3 times)   &              &              &                   &                 &             &               \\
MMS*                     &              &              &                   &                 &             &               \\
Overflow                 &              &              &                   &                 &             &               \\ \bottomrule
\end{tabular}}
\end{table}

